Nucleosynthesis and the Inhomogeneous Chemical Evolution of the Carina Dwarf Galaxy

The detailed abundances of 23 elements in nine bright RGB stars in the Carina dSph are presented based on high resolution spectra gathered at the VLT and Magellan telescopes. A spherical model atmospheres analysis is applied using standard methods to spectra ranging from 380 to 680 nm. The stars in this analysis range from -2.9 < [Fe/H] < -1.3, and adopting the ages determined by Lemasle et al. (2012), we are able to examine the chemical evolution of Carina's old and intermediate-aged populations. One of the main results from this work is the evidence for inhomogeneous mixing in Carina; a large dispersion in [Mg/Fe] indicates poor mixing in the old population, an offset in the [alpha/Fe] ratios between the old and intermediate-aged populations (when examined with previously published results) suggests that the second star formation event occurred in alpha-enriched gas, and one star, Car-612, seems to have formed in a pocket enhanced in SN Ia/II products. This latter star provides the first direct link between the formation of stars with enhanced SN Ia/II ratios in dwarf galaxies to those found in the outer Galactic halo (Ivans et al. 2003). Another important result is the potential evidence for SN II driven winds. We show that the very metal-poor stars in Carina have not been enhanced in AGB or SN Ia products, and therefore their very low ratios of [Sr/Ba] suggests the loss of contributions from the early SNe II. Low ratios of [Na/Fe], [Mn/Fe], and [Cr/Fe] in two of these stars support this scenario, with additional evidence from the low [Zn/Fe] upper limit for one star. It is interesting that the chemistry of the metal-poor stars in Carina is not similar to those in the Galaxy, most of the other dSphs, or the UFDs, and suggests that Carina may be at the critical mass where some chemical enrichment events are lost through SN II driven winds.

==> ngc.BEST.tex <==
\clearpage
\begin{longtable}{lrr|rrrrrr}
\caption[Other Lines List]{Other Lines List} 
 \hline \hline \\ [-1.0ex]
 Wave &  $\chi$ & log~gf & M68 & M68 & M68 & CAR & CAR & CAR \\[0.5ex] \hline
 \\[-1.0ex]
 (\AA) &  (eV) &  & 6022 & 6023 & 6024 & 1087 & 5070 & 7002 \\[0.5ex] \hline
\endfirsthead
 \hline \\[-1.0ex]
 Wave &  $\chi$ & log~gf & N6022 & N6023 & N6024 & 1087 & 5070 & 7002 \\[0.5ex] \hline
 \\[0.5ex]
\endhead
 \\ [-1.0ex] \hline 
\endfoot
 \\[-1.0ex] \hline \hline
\endlastfoot
%\begin{deluxetable}{lrr|rrrrrr}
%\tablecolumns{10}
%\tablewidth{0pt}
%\tablecaption{Other Lines List}
%\tablehead{
%\colhead{Wave} &  \colhead{$\chi$} & \colhead{log~gf} & \colhead{N6022} & \colhead{N6023} & \colhead{N6024} & \colhead{1087} & \colhead{5070} & \colhead{7002}
%}
%\startdata
\\
Fe I \\
 5001.864 & 3.88 & 0.010 & 51.9 & 49.9 & 52.6 & \nodata & \nodata & \nodata \\
 5006.120 & 2.83 & -0.615 & 83.5 & 84.1 & 75.8 & \nodata & \nodata & 70.8 \\
 5012.070 & 0.86 & -2.642 & 122.4 & 117.0 & 121.3 & 138.0 & 184.5 & 134.1 \\
 5014.940 & 3.94 & -0.300 & 35.3 & 38.2 & 42.2 & \nodata & \nodata & \nodata \\
 5022.240 & 3.98 & -0.530 & 35.0 & 36.7 & \nodata & \nodata & \nodata & \nodata \\
 5028.130 & 3.57 & -1.120 & 46.2 & 40.1 & \nodata & \nodata & \nodata & \nodata \\
 5041.072 & 0.96 & -3.086 & 103.3 & \nodata & 91.2 & \nodata & \nodata & \nodata \\
 5041.756 & 1.49 & -2.203 & \nodata & 96.7 & 99.5 & \nodata & \nodata & \nodata \\
 5049.820 & 2.28 & -1.355 & 86.4 & \nodata & 58.4 & \nodata & \nodata & \nodata \\
 5051.635 & 0.92 & -2.764 & 93.3 & 79.3 & 107.7 & \nodata & \nodata & \nodata \\
 5060.080 & 0.00 & -5.460 & \nodata & 49.5 & \nodata & \nodata & \nodata & \nodata \\
 5068.766 & 2.94 & -1.041 & 69.4 & 53.2 & \nodata & \nodata & \nodata & \nodata \\
 5074.750 & 4.22 & -0.200 & 31.1 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 5079.220 & 2.20 & -2.067 & 72.7 & 55.5 & 47.0 & \nodata & \nodata & \nodata \\
 5079.750 & 0.99 & -3.245 & 88.3 & 83.0 & 69.5 & \nodata & \nodata & \nodata \\
 5083.350 & 0.96 & -2.842 & 94.4 & 84.5 & 76.4 & \nodata & 154.1 & 80.3 \\
 5098.700 & 2.18 & -2.030 & 64.6 & 57.8 & 52.0 & \nodata & 123.6 & \nodata \\
 5110.413 & 0.00 & -3.758 & \nodata & 86.0 & \nodata & \nodata & \nodata & \nodata \\
 5123.720 & 1.01 & -3.058 & 90.4 & 87.8 & 75.3 & \nodata & \nodata & \nodata \\
 5127.359 & 0.92 & -3.249 & 86.0 & 96.8 & 75.3 & \nodata & 185.9 & \nodata \\
 5131.470 & 2.22 & -2.510 & 37.1 & 32.4 & 36.2 & \nodata & \nodata & \nodata \\
 5133.690 & 4.18 & 0.140 & \nodata & 31.5 & 44.2 & \nodata & \nodata & \nodata \\
 5137.380 & 4.18 & -0.400 & 37.6 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 5141.740 & 2.42 & -1.964 & \nodata & 37.1 & 34.4 & \nodata & \nodata & \nodata \\
 5142.930 & 0.96 & -3.080 & 95.3 & 91.9 & 85.8 & \nodata & 190.2 & 87.4 \\
 5150.850 & 0.99 & -3.037 & 76.9 & 69.9 & 64.4 & 82.1 & \nodata & 52.4 \\
 5151.920 & 1.01 & -3.321 & 75.1 & 66.5 & 55.0 & 90.0 & \nodata & \nodata \\
 5162.290 & 4.18 & 0.020 & 36.0 & 35.8 & 30.2 & \nodata & \nodata & \nodata \\
 5166.280 & 0.00 & -4.123 & 104.3 & 91.0 & 78.1 & 107.4 & 158.1 & 78.0 \\
 5171.610 & 1.48 & -1.721 & 97.6 & 91.4 & 84.6 & 111.1 & 165.7 & 131.1 \\
 5191.455 & 3.04 & -0.551 & \nodata & 61.1 & 46.2 & \nodata & \nodata & \nodata \\
 5192.340 & 3.00 & -0.421 & 61.5 & 70.6 & 57.3 & \nodata & \nodata & \nodata \\
 5194.942 & 1.56 & -2.021 & 71.3 & 77.9 & 65.8 & 73.9 & 111.7 & \nodata \\
 5198.710 & 2.22 & -2.135 & 32.4 & \nodata & \nodata & 41.1 & \nodata & 44.7 \\
 5202.340 & 2.18 & -1.838 & 77.1 & 71.5 & 69.1 & 41.2 & 133.5 & 74.8 \\
 5204.580 & 0.09 & -4.332 & \nodata & \nodata & \nodata & \nodata & 188.4 & \nodata \\
 5215.190 & 3.27 & -0.930 & 56.3 & 32.0 & \nodata & \nodata & 74.5 & 51.8 \\
 5216.280 & 1.61 & -2.082 & 69.4 & 89.5 & 60.7 & 135.1 & 143.4 & \nodata \\
 5217.390 & 3.21 & -1.160 & 31.2 & 56.3 & \nodata & \nodata & \nodata & \nodata \\
 5225.526 & 0.11 & -4.755 & 53.5 & 46.0 & 42.9 & \nodata & \nodata & 73.0 \\
 5227.190 & 1.56 & -1.227 & 150.8 & 143.1 & 122.5 & 132.3 & \nodata & \nodata \\
 5232.950 & 2.94 & -0.057 & 96.3 & 105.7 & 97.8 & 111.0 & 150.7 & 70.1 \\
 5247.050 & 0.09 & -4.946 & 63.0 & 58.2 & \nodata & \nodata & 49.2 & \nodata \\
 5250.210 & 0.12 & -4.898 & \nodata & 44.4 & \nodata & \nodata & 107.7 & 59.0 \\
 5250.650 & 2.20 & -2.180 & 55.8 & 37.3 & 35.8 & \nodata & \nodata & \nodata \\
 5254.955 & 0.11 & -4.764 & 53.9 & 47.1 & 39.0 & \nodata & \nodata & \nodata \\
 5269.537 & 0.86 & -1.333 & \nodata & \nodata & \nodata & 153.4 & \nodata & 146.2 \\
 5281.790 & 3.04 & -0.833 & 63.3 & 64.2 & 51.7 & 52.6 & \nodata & \nodata \\
 5283.621 & 3.24 & -0.524 & 72.1 & 71.1 & 58.6 & \nodata & 94.4 & \nodata \\
 5302.302 & 3.28 & -0.880 & 59.1 & 50.5 & 50.9 & \nodata & \nodata & 60.8 \\
 5307.370 & 1.61 & -2.912 & 49.7 & 52.9 & 53.2 & 55.8 & \nodata & \nodata \\
 5324.190 & 3.21 & -0.100 & 84.5 & 79.5 & 75.7 & 85.2 & 119.7 & \nodata \\
 5328.039 & 0.92 & -1.465 & 155.9 & 170.4 & 147.6 & 167.6 & \nodata & 162.6 \\
 5328.530 & 1.56 & -1.850 & 111.3 & \nodata & \nodata & 101.0 & \nodata & 84.4 \\
 5332.900 & 1.56 & -2.780 & 49.4 & 49.6 & 49.4 & 50.8 & 93.8 & \nodata \\
 5339.930 & 3.27 & -0.720 & 39.0 & 47.8 & 41.4 & \nodata & \nodata & \nodata \\
 5364.860 & 4.45 & 0.228 & \nodata & \nodata & 30.4 & \nodata & \nodata & \nodata \\
 5367.480 & 4.42 & 0.443 & 42.9 & 37.2 & 36.2 & \nodata & \nodata & \nodata \\
 5369.960 & 4.37 & 0.536 & 43.1 & 46.8 & 39.7 & \nodata & \nodata & \nodata \\
 5371.500 & 0.96 & -1.644 & 156.6 & 152.1 & 154.6 & 186.2 & \nodata & 184.0 \\
 5383.370 & 4.31 & 0.645 & 53.4 & 67.3 & 48.8 & \nodata & \nodata & \nodata \\
 5393.170 & 3.24 & -0.920 & 59.3 & 52.7 & 32.0 & \nodata & \nodata & \nodata \\
 5397.128 & 0.91 & -1.982 & 142.2 & 136.5 & 147.7 & 173.2 & 160.7 & 147.6 \\
 5405.775 & 0.99 & -1.852 & 144.3 & 147.0 & 138.7 & 164.6 & 182.1 & 132.1 \\
 5415.199 & 4.39 & 0.643 & 41.7 & 52.3 & 39.0 & \nodata & \nodata & \nodata \\
 5424.070 & 4.32 & 0.520 & 48.2 & 43.6 & \nodata & 69.0 & 98.1 & \nodata \\
 5429.697 & 0.96 & -1.881 & \nodata & 113.7 & \nodata & 176.8 & \nodata & 106.8 \\
 5434.524 & 1.01 & -2.126 & \nodata & \nodata & \nodata & 110.2 & \nodata & 134.8 \\
 5446.917 & 0.99 & -1.914 & 152.5 & 153.1 & 136.3 & 199.3 & \nodata & 149.5 \\
 5455.609 & 1.01 & -2.091 & \nodata & 167.3 & 155.7 & 149.2 & 200.3 & 114.9 \\
 5497.516 & 1.01 & -2.825 & 101.9 & 101.2 & 89.1 & 90.3 & 156.2 & 86.6 \\
 5501.465 & 0.96 & -3.046 & 102.0 & 104.2 & 90.8 & 121.2 & 137.2 & 95.2 \\
 5506.790 & 0.99 & -2.789 & 98.5 & 97.0 & 87.7 & 103.1 & 193.1 & \nodata \\
 5569.618 & 3.42 & -0.540 & 59.9 & 48.5 & 41.3 & \nodata & 89.9 & 51.4 \\
 5572.842 & 3.40 & -0.310 & 86.4 & 75.5 & 73.6 & \nodata & \nodata & \nodata \\
 5576.089 & 3.43 & -1.000 & 43.3 & 34.1 & \nodata & \nodata & \nodata & \nodata \\
 5586.756 & 3.37 & -0.144 & 68.5 & 74.1 & 66.4 & \nodata & 109.4 & 50.1 \\
 5615.660 & 3.33 & 0.050 & 74.8 & \nodata & 72.0 & 56.0 & 100.7 & 59.4 \\
 5624.540 & 3.42 & -0.755 & 47.0 & 55.9 & 43.9 & \nodata & 118.6 & \nodata \\
 5658.820 & 3.40 & -0.793 & 35.2 & 42.5 & 34.8 & \nodata & 61.2 & \nodata \\
 5701.543 & 2.56 & -2.143 & \nodata & \nodata & \nodata & \nodata & 63.7 & \nodata \\
 5956.693 & 0.86 & -4.498 & \nodata & \nodata & \nodata & \nodata & 60.6 & \nodata \\
 6027.048 & 4.07 & -1.089 & \nodata & \nodata & \nodata & \nodata & 45.2 & \nodata \\
 6056.010 & 4.73 & -0.450 & \nodata & \nodata & \nodata & \nodata & 41.8 & \nodata \\
 6065.481 & 2.61 & -1.410 & 71.7 & 67.0 & 62.7 & \nodata & \nodata & \nodata \\
 6136.615 & 2.45 & -1.410 & 89.7 & 85.6 & 77.3 & 60.3 & 142.7 & 65.7 \\
 6137.691 & 2.59 & -1.346 & 72.4 & 75.1 & 65.1 & 61.2 & 102.2 & 46.0 \\
 6191.558 & 2.43 & -1.416 & 85.5 & 94.6 & 91.5 & 56.0 & 143.8 & 58.9 \\
 6200.312 & 2.61 & -2.373 & \nodata & \nodata & \nodata & \nodata & 58.6 & \nodata \\
 6213.430 & 2.22 & -2.481 & 37.2 & 36.7 & 37.6 & \nodata & \nodata & \nodata \\
 6219.280 & 2.20 & -2.448 & 48.5 & 39.6 & 45.0 & \nodata & 87.7 & \nodata \\
 6230.740 & 2.56 & -1.276 & 92.9 & 87.7 & 87.1 & \nodata & 103.2 & \nodata \\
 6246.320 & 3.60 & -0.733 & 35.5 & \nodata & \nodata & \nodata & 59.2 & \nodata \\
 6252.555 & 2.40 & -1.767 & 80.1 & 83.5 & 65.9 & \nodata & 96.1 & 53.1 \\
 6254.260 & 2.28 & -2.443 & 44.8 & 47.8 & 36.1 & \nodata & 86.1 & \nodata \\
 6265.134 & 2.18 & -2.540 & 41.9 & 45.0 & \nodata & \nodata & 92.4 & \nodata \\
 6297.792 & 2.22 & -2.640 & 51.8 & 57.0 & 49.2 & 52.7 & \nodata & \nodata \\
 6301.500 & 3.65 & -0.720 & 48.3 & 48.2 & \nodata & \nodata & \nodata & \nodata \\
 6335.330 & 2.20 & -2.177 & 55.0 & 66.8 & 57.3 & \nodata & 104.3 & \nodata \\
 6336.820 & 3.69 & -1.050 & 32.7 & 35.9 & \nodata & \nodata & 60.6 & \nodata \\
 6355.029 & 2.84 & -2.291 & \nodata & \nodata & \nodata & \nodata & 66.9 & \nodata \\
 6393.610 & 2.43 & -1.576 & 90.1 & 75.6 & 87.6 & \nodata & 125.9 & 74.1 \\
 6400.000 & 3.60 & -0.290 & 63.5 & 76.5 & 57.1 & \nodata & 123.2 & \nodata \\
 6408.030 & 3.69 & -1.000 & \nodata & \nodata & \nodata & \nodata & 43.2 & \nodata \\
 6411.649 & 3.65 & -0.717 & 38.5 & 44.1 & 35.0 & \nodata & 56.4 & \nodata \\
 6421.350 & 2.28 & -2.014 & 75.0 & 67.8 & 65.5 & 73.7 & 125.0 & 63.7 \\
 6430.846 & 2.18 & -1.946 & 85.3 & 75.5 & 76.1 & \nodata & 142.9 & 58.1 \\
 6481.869 & 2.27 & -3.010 & 32.5 & 33.1 & 30.4 & \nodata & \nodata & \nodata \\
 6494.980 & 2.40 & -1.239 & 98.4 & 101.3 & 91.1 & 72.0 & 124.7 & 89.7 \\
 6592.910 & 2.73 & -1.470 & 55.9 & 64.7 & 43.6 & 58.5 & \nodata & \nodata \\
 6677.990 & 2.69 & -1.420 & 82.1 & 80.9 & 83.6 & 61.4 & 88.7 & 54.0 \\
 6750.150 & 2.42 & -2.621 & 30.5 & \nodata & \nodata & \nodata & \nodata & \nodata \\
\\
Fe II \\
 4178.860 & 2.57 & -2.530 & 64.0 & 69.6 & 52.1 & \nodata & 99.2 & 71.6 \\
 4233.170 & 2.57 & -2.000 & 79.0 & \nodata & 76.4 & 100.5 & 127.0 & 101.0 \\
 4416.830 & 2.78 & -2.610 & 62.8 & 60.8 & 62.4 & 49.5 & \nodata & \nodata \\
 4489.180 & 2.83 & -2.970 & 39.0 & 43.5 & 36.6 & \nodata & \nodata & \nodata \\
 4491.400 & 2.86 & -2.690 & 45.1 & 44.3 & 45.8 & \nodata & \nodata & \nodata \\
 4508.290 & 2.86 & -2.220 & 70.7 & 71.5 & 63.7 & \nodata & 95.7 & \nodata \\
 4515.340 & 2.84 & -2.480 & 68.6 & \nodata & 62.6 & \nodata & 65.5 & \nodata \\
 4520.220 & 2.81 & -2.610 & 63.5 & 61.5 & 51.6 & \nodata & \nodata & 40.0 \\
 4541.520 & 2.86 & -3.050 & 40.2 & 39.8 & 39.5 & \nodata & \nodata & \nodata \\
 4555.890 & 2.83 & -2.280 & 56.5 & 66.1 & \nodata & \nodata & 78.4 & \nodata \\
 4576.340 & 2.84 & -3.040 & 38.9 & 41.1 & 41.1 & \nodata & \nodata & \nodata \\
 4582.840 & 2.84 & -3.090 & \nodata & 36.1 & 37.7 & \nodata & 50.7 & 49.1 \\
 4583.830 & 2.81 & -2.020 & 89.5 & 100.7 & \nodata & 92.4 & \nodata & \nodata \\
 4629.340 & 2.81 & -2.380 & 70.3 & 64.8 & 60.5 & 47.8 & 98.4 & 50.5 \\
 4731.450 & 2.89 & -3.370 & 33.1 & \nodata & 34.3 & \nodata & 50.6 & \nodata \\
 4923.920 & 2.89 & -1.320 & 92.9 & 112.4 & 103.0 & 117.4 & 164.3 & \nodata \\
 5018.430 & 2.89 & -1.220 & 116.1 & 117.3 & 119.0 & 131.0 & 131.1 & 89.7 \\
 5197.570 & 3.23 & -2.100 & \nodata & 45.7 & \nodata & 51.5 & \nodata & \nodata \\
 5234.630 & 3.22 & -2.118 & 57.2 & 53.8 & 48.8 & \nodata & \nodata & \nodata \\
 5276.000 & 3.20 & -1.950 & \nodata & 43.2 & \nodata & \nodata & 43.5 & \nodata \\
 5284.100 & 2.89 & -3.190 & 34.2 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 5534.850 & 3.24 & -2.920 & 30.9 & 34.7 & 41.2 & \nodata & \nodata & \nodata \\
 6516.080 & 2.89 & -3.450 & \nodata & 31.9 & \nodata & \nodata & \nodata & \nodata \\
\\
O I \\
 6300.310 & 0.00 & -9.750 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Na I \\
 5688.210 & 2.10 & -0.370 & \nodata & 32 S & \nodata & \nodata & \nodata & \nodata \\
 5889.970 & 0.00 & 0.110  & 231 S  & 227 S & 194 S & 110 S & 240 S & 170 S \\
 5895.924 & 0.00 & -0.190 & 200 S  & 198 S & 158 S & 134 S & 245 S & 172 S\\
\\
Mg I \\
 3829.355 & 2.71 & -0.210 & 180 S & 160 S & 169 S & \nodata & \nodata & \nodata \\
 3832.304 & 2.71 & 0.150 & 187 S & 173 S & 200 S & \nodata & \nodata & \nodata \\
 5172.700 & 2.71 & -0.380 & 190 S & 167 S & 185 S & \nodata & \nodata & 200 S \\
 5528.410 & 4.34 & -0.480 & 55.0 & 40.8 & 39.9 & 83.0 & 74.4 & 55.0 \\
\\
Si I \\
 5684.520 & 4.93 & -1.650 & \nodata & \nodata & \nodata & $<$40.0 & $<$40.0 & $<$40.0 \\
 6155.140 & 5.62 & -0.800 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Ca I \\
 4318.660 & 1.90 & -0.210 & 78.1 & 79.2 & 75.9 & \nodata & \nodata & \nodata \\
 4425.440 & 1.88 & -0.360 & 78.1 & 73.8 & 79.2 & \nodata & 55.8 & \nodata \\
 4435.680 & 1.89 & -0.520 & 82.3 & 75.3 & 87.4 & \nodata & 71.0 & \nodata \\
 4454.790 & 1.90 & 0.260 & 109.7 & 105.9 & 108.4 & \nodata & 116.0 & \nodata \\
 4455.890 & 1.90 & -0.530 & 68.2 & 62.6 & 61.6 & \nodata & 105.3 & \nodata \\
 5588.749 & 2.52 & 0.210 & 70.0 & 68.6 & 61.6 & \nodata & 62.3 & 44.4 \\
 5594.470 & 2.52 & 0.097 & 56.0 & 60.8 & 49.6 & \nodata & 85.3 & \nodata \\
 5598.490 & 2.52 & -0.087 & 45.0 & 45.9 & 40.4 & \nodata & 75.5 & 47.7 \\
 5857.451 & 2.93 & 0.230 & 43.6 & 52.9 & 34.8 & \nodata & \nodata & \nodata \\
 6102.730 & 1.88 & -0.790 & 69.0 & 49.4 & 57.7 & \nodata & \nodata & 40.0 \\
 6122.230 & 1.89 & -0.320 & 93.5 & 95.4 & 85.3 & 40.0 & \nodata & 40.0 \\
 6162.173 & 1.90 & -0.090 & 101.1 & 116.2 & 97.4 & 52.7 & \nodata & 54.6 \\
 6169.560 & 2.52 & -0.480 & 44.1 & 33.7 & \nodata & \nodata & \nodata & \nodata \\
 6439.080 & 2.52 & 0.390 & 91.3 & 89.1 & 76.2 & 65.1 & 88.7 & 49.6 \\
 6449.810 & 2.52 & -0.502 & \nodata & 34.5 & 45.7 & \nodata & 58.0 & \nodata \\
 6471.670 & 2.52 & -0.760 & 33.4 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 6493.790 & 2.52 & -0.320 & 61.4 & 54.6 & 53.1 & \nodata & \nodata & \nodata \\
 6717.681 & 2.71 & -0.610 & 36.3 & \nodata & \nodata & \nodata & \nodata & \nodata \\
\\
Sc II \\
 4246.822 & 0.32 & 0.240 & 148.4 & 140.0 & 140.2 & \nodata & 130.3 & \nodata \\
 4314.083 & 0.62 & -0.100 & 132.9 & 132.4 & 123.2 & 120.4 & 186.1 & \nodata \\
 4320.730 & 0.60 & -0.260 & \nodata & \nodata & \nodata & 78.0 & \nodata & \nodata \\
 4325.000 & 0.60 & -0.440 & 113.3 & 77.6 & 104.8 & \nodata & 93.1 & 87.6 \\
 4400.389 & 0.61 & -0.540 & 104.7 & 107.9 & 94.6 & 85.6 & 100.1 & 88.5 \\
 4415.560 & 0.60 & -0.640 & 89.7 & 93.4 & 87.8 & \nodata & 79.1 & 66.2 \\
 4670.410 & 1.36 & -0.580 & 47.1 & 49.8 & 46.6 & \nodata & \nodata & 60.1 \\
 5031.021 & 1.36 & -0.400 & 66.8 & 67.7 & 62.3 & \nodata & \nodata & \nodata \\
 5239.810 & 1.46 & -0.770 & 44.2 & 36.3 & 33.1 & \nodata & \nodata & \nodata \\
 5526.790 & 1.77 & 0.030 & \nodata & 31.3 & \nodata & 54.1 & \nodata & \nodata \\
 5657.910 & 1.51 & -0.600 & 54.9 & 55.4 & 50.0 & 52.1 & 67.8 & \nodata \\
 5667.160 & 1.50 & -1.310 & \nodata & \nodata & \nodata & \nodata & 65.2 & \nodata \\
 5684.210 & 1.51 & -1.070 & 39.4 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 6604.580 & 1.36 & -1.310 & \nodata & \nodata & \nodata & \nodata & 56.1 & \nodata \\
\\
Ti I \\
 3904.780 & 0.90 & 0.030 & \nodata & 33.9 & \nodata & \nodata & \nodata & \nodata \\
 3924.530 & 0.02 & -0.881 & \nodata & 34.6 & \nodata & \nodata & \nodata & \nodata \\
 3958.220 & 0.05 & -0.160 & \nodata & 80.9 & 89.2 & \nodata & \nodata & \nodata \\
 3989.760 & 0.02 & -0.142 & 73.0 & 75.1 & 90.1 & 92.2 & \nodata & \nodata \\
 3998.640 & 0.05 & -0.050 & 66.4 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 4008.930 & 0.02 & -1.016 & \nodata & 61.2 & 51.8 & \nodata & \nodata & \nodata \\
 4512.730 & 0.84 & -0.424 & 35.3 & \nodata & 31.3 & \nodata & \nodata & \nodata \\
 4533.250 & 0.85 & 0.480 & 83.3 & 70.9 & 66.4 & \nodata & 51.7 & \nodata \\
 4534.780 & 0.84 & 0.280 & 70.5 & 62.0 & 57.9 & \nodata & \nodata & 40.0 \\
 4535.570 & 0.83 & 0.120 & 60.8 & 59.4 & 59.3 & \nodata & \nodata & 40.7 \\
 4544.690 & 0.82 & -0.520 & 35.8 & \nodata & \nodata & \nodata & 56.9 & \nodata \\
 4548.760 & 0.83 & -0.298 & 38.9 & 40.8 & \nodata & \nodata & \nodata & \nodata \\
 4681.910 & 0.05 & -1.015 & 54.0 & 47.4 & 49.5 & \nodata & 108.6 & \nodata \\
 4840.870 & 0.90 & -0.450 & 30.1 & \nodata & \nodata & 46.9 & \nodata & \nodata \\
 4981.731 & 0.84 & 0.500 & 77.6 & 70.5 & 69.1 & \nodata & 101.3 & \nodata \\
 4991.065 & 0.84 & 0.380 & 78.4 & 77.4 & 88.6 & \nodata & \nodata & \nodata \\
 4999.503 & 0.83 & 0.250 & 61.6 & 60.2 & 38.2 & 84.4 & 66.0 & \nodata \\
 5007.210 & 0.82 & 0.168 & 79.9 & 76.0 & 95.6 & \nodata & 114.3 & \nodata \\
 5016.160 & 0.85 & -0.510 & \nodata & 35.5 & \nodata & \nodata & \nodata & \nodata \\
 5020.020 & 0.84 & -0.358 & 50.2 & \nodata & 34.4 & \nodata & \nodata & \nodata \\
 5024.840 & 0.82 & -0.546 & 37.8 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 5035.900 & 1.46 & 0.260 & 35.0 & 32.4 & 39.6 & \nodata & \nodata & \nodata \\
 5036.460 & 1.44 & 0.186 & 32.4 & 33.9 & 45.0 & \nodata & \nodata & \nodata \\
 5038.400 & 1.43 & 0.069 & \nodata & \nodata & 30.3 & \nodata & \nodata & \nodata \\
 5039.957 & 0.02 & -1.130 & 50.9 & 49.3 & 45.9 & \nodata & 119.2 & \nodata \\
 5064.650 & 0.05 & -0.930 & 49.7 & 46.4 & 44.1 & \nodata & \nodata & \nodata \\
 5173.743 & 0.00 & -1.120 & 52.7 & 41.0 & 30.4 & \nodata & 85.4 & \nodata \\
 5192.969 & 0.02 & -1.010 & 31.3 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 5210.390 & 0.05 & -0.580 & 45.4 & 81.5 & 39.1 & 133.4 & \nodata & 72.1 \\
\\
Ti II \\
 3813.390 & 0.61 & -2.020 & 93.6 & 68.4 & 98.2 & \nodata & \nodata & \nodata \\
 3882.290 & 1.12 & -1.710 & \nodata & 79.5 & \nodata & \nodata & \nodata & \nodata \\
 3900.540 & 1.13 & -0.450 & \nodata & \nodata & 110.7 & \nodata & \nodata & \nodata \\
 3913.468 & 1.12 & -0.530 & 167.2 & \nodata & 143.7 & \nodata & \nodata & \nodata \\
 3987.610 & 0.61 & -2.730 & 58.1 & 48.8 & 53.0 & \nodata & \nodata & \nodata \\
 4012.385 & 0.57 & -1.610 & 111.5 & 105.6 & 108.7 & \nodata & \nodata & \nodata \\
 4025.120 & 0.61 & -1.980 & 85.7 & 90.2 & 86.5 & \nodata & \nodata & \nodata \\
 4028.343 & 1.89 & -1.000 & 55.0 & 63.8 & 70.8 & \nodata & \nodata & \nodata \\
 4053.830 & 1.89 & -1.210 & 54.7 & 53.3 & \nodata & 77.5 & \nodata & \nodata \\
 4161.530 & 1.08 & -2.160 & 40.8 & 71.1 & 64.3 & \nodata & \nodata & \nodata \\
 4163.630 & 2.59 & -0.400 & 59.8 & 65.9 & 55.8 & \nodata & \nodata & \nodata \\
 4184.310 & 1.08 & -2.510 & \nodata & 41.6 & \nodata & \nodata & 85.3 & \nodata \\
 4290.219 & 1.16 & -1.120 & 126.6 & 124.0 & 123.1 & 108.5 & 123.8 & 106.4 \\
 4300.049 & 1.18 & -0.770 & 149.8 & 134.9 & 135.4 & \nodata & 102.4 & \nodata \\
 4301.930 & 1.16 & -1.200 & \nodata & 73.2 & 76.0 & 88.0 & 93.1 & 114.7 \\
 4312.860 & 1.18 & -1.160 & 140.2 & 125.9 & \nodata & 90.6 & 159.6 & \nodata \\
 4330.720 & 1.18 & -2.060 & 73.6 & 58.7 & 55.0 & 41.9 & 90.1 & 60.9 \\
 4337.880 & 1.08 & -1.130 & 128.7 & 122.7 & 118.1 & 100.3 & \nodata & 110.0 \\
 4395.850 & 1.24 & -2.170 & 73.2 & 72.5 & 62.4 & 42.5 & 90.8 & \nodata \\
 4399.770 & 1.24 & -1.290 & 124.1 & 114.0 & 106.9 & 107.2 & 94.0 & \nodata \\
 4407.680 & 1.22 & -2.470 & 81.2 & 78.3 & 74.0 & 77.2 & \nodata & \nodata \\
 4417.719 & 1.16 & -1.430 & 114.1 & 110.1 & 109.5 & \nodata & 115.0 & \nodata \\
 4418.330 & 1.24 & -2.450 & 66.8 & 63.2 & 61.5 & 51.5 & 69.4 & 66.6 \\
 4441.730 & 1.18 & -2.410 & 49.1 & 43.5 & \nodata & 40.0 & 55.7 & \nodata \\
 4443.794 & 1.08 & -0.710 & 122.1 & 104.6 & 100.8 & 138.0 & 158.0 & 107.7 \\
 4444.560 & 1.12 & -2.030 & 72.5 & 68.4 & 61.2 & \nodata & 48.2 & \nodata \\
 4450.482 & 1.08 & -1.450 & 103.3 & 103.2 & 98.2 & 92.3 & 128.0 & 61.5 \\
 4464.450 & 1.16 & -2.080 & 91.2 & 72.0 & 80.0 & 58.1 & \nodata & 55.2 \\
 4468.507 & 1.13 & -0.620 & 121.8 & 131.6 & 128.0 & 131.3 & \nodata & 113.3 \\
 4469.140 & 1.08 & -2.870 & 64.1 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 4470.860 & 1.16 & -2.280 & 75.4 & 71.1 & 65.6 & \nodata & 58.9 & 38.7 \\
 4493.510 & 1.08 & -2.740 & 36.8 & 31.5 & 39.8 & \nodata & \nodata & \nodata \\
 4501.273 & 1.12 & -0.750 & 140.0 & 140.4 & 136.3 & 108.9 & 150.4 & 124.5 \\
 4518.330 & 1.08 & -2.560 & 61.7 & 55.1 & 56.6 & \nodata & 39.1 & 58.0 \\
 4529.470 & 1.57 & -2.040 & 56.3 & 55.9 & 56.9 & \nodata & 56.6 & \nodata \\
 4533.969 & 1.24 & -0.770 & 150.8 & 146.0 & 138.4 & 118.8 & 178.0 & 88.2 \\
 4544.030 & 1.24 & -2.410 & 44.5 & 38.3 & \nodata & \nodata & \nodata & \nodata \\
 4545.140 & 1.13 & -1.810 & \nodata & 51.2 & 45.7 & \nodata & \nodata & \nodata \\
 4563.761 & 1.22 & -0.960 & 132.3 & 135.5 & 123.6 & 131.9 & 171.2 & 110.6 \\
 4568.310 & 1.22 & -2.650 & \nodata & 31.6 & \nodata & \nodata & \nodata & \nodata \\
 4571.968 & 1.57 & -0.520 & 139.5 & 141.2 & 127.5 & 140.7 & 148.8 & 100.3 \\
 4583.410 & 1.17 & -2.870 & 30.6 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 4589.960 & 1.24 & -1.780 & 84.4 & 89.0 & 83.2 & 75.6 & 94.5 & \nodata \\
 4657.210 & 1.24 & -2.320 & 58.3 & 57.2 & 52.2 & \nodata & 67.8 & \nodata \\
 4708.670 & 1.24 & -2.210 & 47.9 & 51.9 & 37.1 & 58.4 & 62.8 & \nodata \\
 4763.880 & 1.22 & -2.450 & 55.6 & 47.4 & 48.0 & \nodata & 74.9 & \nodata \\
 4779.990 & 2.05 & -1.370 & 62.6 & 50.2 & 50.2 & \nodata & 77.5 & 49.7 \\
 4798.530 & 1.08 & -2.670 & 38.0 & 32.0 & 44.9 & \nodata & 65.0 & \nodata \\
 4805.090 & 2.06 & -1.120 & 69.9 & \nodata & 64.4 & 59.4 & 69.3 & 40.0 \\
 4865.612 & 1.12 & -2.590 & 52.4 & \nodata & 45.6 & \nodata & \nodata & 52.4 \\
 4911.180 & 3.12 & -0.340 & \nodata & \nodata & \nodata & \nodata & 68.4 & \nodata \\
 5129.160 & 1.89 & -1.390 & 60.8 & 59.0 & 65.8 & \nodata & \nodata & \nodata \\
 5154.070 & 1.57 & -1.520 & 55.9 & 54.4 & \nodata & \nodata & \nodata & \nodata \\
 5185.913 & 1.89 & -1.350 & 36.2 & \nodata & \nodata & \nodata & \nodata & \nodata \\
 5188.680 & 1.58 & -1.220 & \nodata & \nodata & 44.3 & 123.4 & \nodata & \nodata \\
 5226.550 & 1.57 & -1.000 & 108.7 & 85.9 & 83.9 & \nodata & \nodata & \nodata \\
 5336.771 & 1.58 & -1.700 & 52.8 & 51.8 & 53.2 & 86.3 & \nodata & 50.8 \\
 5381.010 & 1.57 & -1.780 & 47.0 & 53.0 & 48.0 & \nodata & \nodata & \nodata \\
 5418.770 & 1.58 & -2.110 & 35.5 & 31.1 & \nodata & \nodata & 47.8 & 51.3 \\
 6559.588 & 2.05 & -2.019 & 34.8 & 33.7 & \nodata & \nodata & \nodata & \nodata \\
\\
V I \\
 4111.770 & 0.30 & 0.408 & 41.9 & 36.3 & 38.8 & \nodata & \nodata & \nodata \\
 4379.230 & 0.55 & 0.301 & 43.0 & 49.2 & 36.3 & 61.0 & 43.3 & \nodata \\
\\
Cr I \\
 4254.332 & 0.00 & -0.110 & \nodata & 109.0 & \nodata & 125.0 & \nodata & 124.7 \\
 4274.796 & 0.00 & -0.230 & 120.4 & 118.4 & 111.6 & 102.0 & \nodata & \nodata \\
 4289.720 & 0.00 & -0.360 & 125.0 & 125.2 & 117.6 & 97.0 & \nodata & 100.5 \\
 4496.840 & 0.94 & -1.150 & 47.3 & 68.4 & 48.5 & \nodata & 54.4 & \nodata \\
 4600.750 & 1.00 & -1.260 & 33.2 & 29.9 & \nodata & \nodata & \nodata & \nodata \\
 4616.140 & 0.98 & -1.190 & 44.9 & 36.1 & 37.3 & \nodata & 71.4 & 48.5 \\
 4626.190 & 0.97 & -1.320 & 37.1 & 35.9 & 31.7 & \nodata & 44.1 & \nodata \\
 4646.170 & 1.03 & -0.700 & 68.6 & 51.1 & \nodata & \nodata & \nodata & \nodata \\
 4652.160 & 1.00 & -1.030 & 62.4 & 43.4 & 43.3 & \nodata & 69.2 & \nodata \\
 5206.040 & 0.94 & 0.019 & 110.3 & 103.6 & 93.8 & \nodata & 168.1 & 95.7 \\
 5208.419 & 0.94 & 0.160 & 135.3 & 142.0 & 126.3 & \nodata & \nodata & \nodata \\
 5345.801 & 1.00 & -0.980 & 40.6 & \nodata & \nodata & \nodata & 59.9 & \nodata \\
 5409.800 & 1.03 & -0.720 & 74.2 & 55.5 & 56.6 & 53.6 & 71.9 & \nodata \\
%\\
%Cr II \\
% 4558.650 & 4.07 & -0.660 & 40.5 & 42.6 & 29.7 & $<$40.0 & 50.0 & $<$40.0 \\
% 4824.130 & 3.87 & -1.230 & 39.2 & 36.3 & 32.6 & \nodata & \nodata & \nodata \\
\\
Mn I \\
 4030.753 & 0.00 & -0.480 & 139.9 & 135.6 & 151.7 & \nodata & \nodata & \nodata \\
 4033.062 & 0.00 & -0.620 & 128.6 & 96.5 & 114.9 & 118.3 & 125.6 & 143.7 \\
 4034.483 & 0.00 & -0.810 & 118.2 & 106.0 & 108.6 & 102.6 & 124.2 & 94.4 \\
 4041.360 & 2.11 & 0.285 & 47.3 & 52.1 & \nodata & \nodata & 59.0 & \nodata \\
 4754.040 & 2.28 & -0.090 & 33.3 & 30.0 & \nodata & \nodata & \nodata & \nodata \\
 4783.430 & 2.30 & 0.042 & 33.7 & 35.6 & 30.7 & \nodata & \nodata & \nodata \\
 4823.524 & 2.32 & 0.140 & 46.6 & 39.5 & \nodata & \nodata & \nodata & \nodata \\
\\
Co I \\
 3842.050 & 0.92 & -0.770 & 63.8 & 57.6 & 70.9 & \nodata & \nodata & \nodata \\
 3845.470 & 0.92 & 0.010 & 80.9 & 85.8 & \nodata & \nodata & \nodata & \nodata \\
 3873.120 & 0.43 & -0.660 & \nodata & 115.3 & 128.9 & \nodata & \nodata & \nodata \\
 3881.870 & 0.58 & -1.130 & 77.8 & 73.1 & 75.8 & \nodata & \nodata & \nodata \\
 3995.302 & 0.92 & -0.220 & 76.8 & \nodata & \nodata & \nodata & \nodata & 65.2 \\
 4020.900 & 0.43 & -2.070 & \nodata & 37.0 & 49.0 & \nodata & \nodata & \nodata \\
 4110.530 & 1.05 & -1.080 & 64.5 & 53.7 & 49.8 & \nodata & \nodata & \nodata \\
 4118.767 & 1.05 & -0.490 & \nodata & \nodata & 109.2 & \nodata & \nodata & \nodata \\
 4121.311 & 0.92 & -0.320 & 101.2 & 88.9 & 98.5 & \nodata & \nodata & 101.1 \\
 5483.34  & 1.71 & -1.488 & \nodata & \nodata & \nodata & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Ni I \\
 3807.138 & 0.42 & -1.180 & \nodata & 114.4 & 95.7 & \nodata & \nodata & \nodata \\
 4401.550 & 3.19 & 0.084 & 56.9 & 58.8 & 50.8 & \nodata & \nodata & 54.5 \\
 4714.420 & 3.38 & 0.230 & 44.1 & 44.0 & 44.0 & 54.9 & 52.5 & 43.4 \\
 5035.370 & 3.63 & 0.290 & 33.8 & \nodata & 38.6 & \nodata & \nodata & \nodata \\
 5080.520 & 3.65 & 0.130 & \nodata & 49.2 & \nodata & \nodata & \nodata & \nodata \\
 5084.080 & 3.68 & 0.030 & 30.4 & \nodata & \nodata & \nodata & 55.0 & \nodata \\
 5137.070 & 1.68 & -1.990 & 43.3 & 74.6 & 53.5 & \nodata & \nodata & \nodata \\
 5476.920 & 1.83 & -0.890 & 89.4 & 98.2 & 75.0 & \nodata & 177.0 & 95.8 \\
 5578.730 & 1.68 & -2.670 & \nodata & \nodata & \nodata & \nodata & 59.9 & \nodata \\
 6327.600 & 1.68 & -3.090 & \nodata & \nodata & \nodata & \nodata & 53.2 & \nodata \\
 6643.640 & 1.68 & -2.300 & 39.1 & 43.0 & \nodata & \nodata & 56.5 & \nodata \\
 6767.780 & 1.83 & -2.170 & 37.3 & 45.9 & 35.0 & \nodata & 68.7 & \nodata \\
\\
Cu I \\
 5105.500 & 1.39 & -1.505 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Zn I \\
 4722.153 & 4.03 & -0.338 & 28.7 & 25.1 & \nodata & \nodata & \nodata & \nodata \\
 4810.540 & 4.08 & -0.170 & 36.8 & 36.9 & 28.5 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Sr II \\
 4077.710 & 0.00 & 0.170 & 162.1 & 151.1 & 155.5  &  S & S & S  \\
 4215.520 & 0.00 & -0.140 & 162.6 & 144.2 & 138.0 &  S & S & 84 S \\
\\
Y II \\
 3950.360 & 0.10 & -0.490 & \nodata & 43.1 & 46.5 & \nodata & \nodata & \nodata \\
 4883.690 & 1.08 & 0.070 & 38.4 & 32.0 & 30.4 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Zr II \\
 4208.980 & 0.71 & -0.460 & 41.0 & 29.9 & 25.7 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Ba II \\
 4554.030 & 0.00 & 0.170  & 140.7 & 127.5 & 147.5 & S     & 135.5 & 81.9 \\
 5853.690 & 0.60 & -1.010 & 56.2  & 49.9  & 54.6  & $<$30 & $<$30 & $<$30 \\
 6141.730 & 0.70 & -0.077 & 106.3 & 103.2 & 111.6 & S    & 93.4   & 41.2 \\
 6496.910 & 0.60 & -0.380 & 106.5 & 102.4 & 101.5 & 47.5 & S      & 50.3 \\
\\
La II \\
 6320.430 & 0.17 & -1.562 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
 6390.460 & 0.32 & -1.400 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
 6774.270 & 0.13 & -1.708 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
\\
Eu II \\
 4129.700 & 0.00 & 0.220 &  \nodata & 64.0    & 69.6    & $<$40   & 66 S     & $<$40  \\
 4205.040 & 0.00 & 0.210 &       S  & 69.7    & 65.3    & $<$40   &    S     & $<$40  \\
 6645.130 & 1.37 & 0.120 & $<$30 & $<$30 & $<$30        & $<$40   &  $<$ 40  & $<$40  \\
\\
Nd II \\
 5319.820 & 0.55 & -0.140 & $<$30.0 & $<$30.0 & $<$30.0 & $<$40.0 & $<$40.0 & $<$40.0 \\
 \\
%\enddata
%\tablecomments{  }
%\end{deluxetable}
\end{longtable}



==> ukv.BEST.tex <==
\clearpage
\begin{longtable}{lrr|rrrrrr}
\caption[]{Machine Readable Version Only} \\
 \hline \hline \\[-1.0ex]
 Wave &  $\chi$ & log~gf & CAR & CAR & CAR & CAR & CAR & CAR \\[0.5ex] \hline
 \\[-1.0ex]
 (\AA) &  (eV) &  & 484 & 524 & 612 & 705 & 769 & 1013  \\[0.5ex] \hline
\endfirsthead
 \hline \\[-1.0ex]
 Wave &  $\chi$ & log~gf & 484 & 524 & 612 & 705 & 769 & 1013  \\[0.5ex] \hline
 \\[0.5ex]
\endhead
 \\ [-1.0ex] \hline 
\endfoot
 \\[-1.0ex] \hline \hline
\endlastfoot

%\begin{deluxetable}{lrr|rrrrrr}
%\rotate{}
%\tablecolumns{10}
%\tablewidth{0pt}
%\tablecaption{Other Lines List}
%\tablehead{
%\colhead{Wave} & \colhead{$\chi$} & \colhead{log~gf} & \colhead{484} & \colhead{524} & \colhead{612} & \colhead{705} & \colhead{769} & \colhead{1013}
%}
%\startdata
\\
Fe I \\
 5001.864 & 3.88 & 0.010 & 124.9 & 116.7 & 124.0 & 134.0 & 104.3 & 165.1 \\
 5006.120 & 2.83 & -0.615 & 194.7 & 166.1 & 185.2 & 193.8 & 158.2 & \nodata \\
 5012.070 & 0.86 & -2.642 & \nodata & 195.0 & \nodata & \nodata & 179.3 & \nodata \\
 5014.940 & 3.94 & -0.300 & 113.4 & 103.4 & 117.0 & 114.3 & 65.4 & 97.2 \\
 5022.240 & 3.98 & -0.530 & 84.6 & 84.0 & 107.4 & 101.8 & 75.9 & 126.5 \\
 5028.130 & 3.57 & -1.120 & 96.3 & 75.5 & 94.5 & 91.5 & 54.6 & 83.1 \\
 5041.072 & 0.96 & -3.086 & \nodata & \nodata & 154.1 & \nodata & \nodata & \nodata \\
 5044.210 & 2.85 & -2.040 & 120.5 & 99.5 & 107.0 & 95.3 & 76.2 & 73.9 \\
 5049.820 & 2.28 & -1.355 & 194.3 & 171.2 & 190.9 & 189.1 & 163.9 & 180.5 \\
 5051.635 & 0.92 & -2.764 & \nodata & 196.3 & 191.9 & \nodata & 176.6 & \nodata \\
 5060.080 & 0.00 & -5.460 & \nodata & 135.3 & 148.8 & 154.4 & 138.8 & \nodata \\
 5068.766 & 2.94 & -1.041 & 165.0 & 139.8 & 146.1 & 179.4 & 137.4 & 158.4 \\
 5074.750 & 4.22 & -0.200 & 117.7 & 87.2 & 117.5 & 108.8 & 98.0 & 116.3 \\
 5079.220 & 2.20 & -2.067 & 154.0 & 141.5 & 147.8 & 140.7 & 125.1 & 116.0 \\
 5079.750 & 0.99 & -3.245 & \nodata & 180.5 & 173.7 & \nodata & 169.2 & \nodata \\
 5080.950 & 3.27 & -3.090 & \nodata & \nodata & \nodata & \nodata & \nodata & 41.2 \\
 5083.350 & 0.96 & -2.842 & \nodata & 181.2 & 184.5 & 197.5 & 177.4 & \nodata \\
 5090.770 & 4.26 & -0.360 & 91.8 & 80.1 & 95.6 & 98.5 & 61.6 & 74.1 \\
 5098.700 & 2.18 & -2.030 & \nodata & 172.5 & \nodata & \nodata & \nodata & 157.6 \\
 5110.413 & 0.00 & -3.758 & \nodata & \nodata & \nodata & \nodata & 197.3 & \nodata \\
 5123.720 & 1.01 & -3.058 & 180.4 & 186.4 & 197.7 & 189.0 & 191.1 & 197.2 \\
 5125.120 & 4.22 & -0.140 & 107.3 & 99.9 & 122.3 & 123.7 & 103.7 & 126.3 \\
 5127.359 & 0.92 & -3.249 & \nodata & 177.6 & 184.9 & \nodata & 152.3 & 189.7 \\
 5131.470 & 2.22 & -2.510 & 150.9 & 112.9 & 124.0 & 146.9 & 112.6 & 172.1 \\
 5133.690 & 4.18 & 0.140 & 140.7 & 130.6 & 141.6 & 139.7 & 128.1 & 153.8 \\
 5137.380 & 4.18 & -0.400 & 105.0 & 93.9 & \nodata & 108.3 & 72.1 & 113.4 \\
 5141.740 & 2.42 & -1.964 & 135.8 & 109.8 & 123.4 & 138.2 & 113.2 & 133.1 \\
 5150.850 & 0.99 & -3.037 & \nodata & 177.4 & 194.0 & 187.6 & 169.2 & 170.0 \\
 5151.920 & 1.01 & -3.321 & \nodata & 162.6 & 186.1 & 186.8 & 160.5 & \nodata \\
 5159.050 & 4.28 & -0.810 & 55.7 & 36.8 & 74.5 & 69.9 & 44.9 & 53.1 \\
 5162.290 & 4.18 & 0.020 & 148.2 & 115.7 & 140.3 & 131.0 & 131.6 & \nodata \\
 5165.410 & 4.22 & -0.040 & 89.6 & 64.5 & 86.3 & 77.4 & 67.8 & 71.0 \\
 5166.280 & 0.00 & -4.123 & \nodata & 192.4 & \nodata & 199.5 & 169.8 & \nodata \\
 5171.610 & 1.48 & -1.721 & \nodata & \nodata & \nodata & \nodata & 180.0 & 197.9 \\
 5191.455 & 3.04 & -0.551 & \nodata & 166.3 & 190.3 & \nodata & 159.3 & \nodata \\
 5192.340 & 3.00 & -0.421 & 198.6 & 169.6 & 179.4 & 173.9 & 158.2 & 195.1 \\
 5194.942 & 1.56 & -2.021 & \nodata & 200.1 & \nodata & 184.2 & 160.3 & \nodata \\
 5198.710 & 2.22 & -2.135 & 165.6 & 148.7 & 164.3 & 141.1 & 146.6 & 178.8 \\
 5202.340 & 2.18 & -1.838 & \nodata & 168.9 & 181.5 & 195.7 & 140.5 & 200.4 \\
 5215.190 & 3.27 & -0.930 & 132.0 & 111.9 & 123.7 & 130.1 & 109.2 & 133.2 \\
 5216.280 & 1.61 & -2.082 & \nodata & 189.1 & \nodata & \nodata & 158.7 & 191.4 \\
 5217.390 & 3.21 & -1.160 & 127.2 & 121.9 & 116.2 & 117.0 & 112.7 & 103.6 \\
 5225.526 & 0.11 & -4.755 & \nodata & 164.0 & 174.2 & 174.1 & 158.5 & 178.7 \\
 5232.950 & 2.94 & -0.057 & \nodata & 187.0 & \nodata & \nodata & \nodata & 175.1 \\
 5242.490 & 3.63 & -0.970 & 106.3 & 84.5 & 112.6 & \nodata & 77.2 & 111.5 \\
 5247.050 & 0.09 & -4.946 & \nodata & 176.5 & 168.5 & \nodata & 172.8 & \nodata \\
 5250.210 & 0.12 & -4.898 & \nodata & 163.8 & 188.7 & \nodata & 161.6 & 176.5 \\
 5250.650 & 2.20 & -2.180 & 193.9 & 162.5 & 150.7 & 191.9 & 143.6 & \nodata \\
 5253.020 & 2.28 & -3.810 & 34.8 & \nodata & 53.7 & 46.1 & \nodata & 42.8 \\
 5254.955 & 0.11 & -4.764 & \nodata & 189.4 & 170.7 & \nodata & 162.9 & 194.3 \\
 5263.310 & 3.27 & -0.879 & 147.4 & 120.3 & 146.8 & 137.8 & 120.9 & 125.3 \\
 5266.555 & 3.00 & -0.385 & 180.8 & 166.9 & 184.8 & 168.0 & 162.9 & 156.3 \\
 5281.790 & 3.04 & -0.833 & 184.4 & 141.4 & 169.7 & 142.5 & 137.0 & 142.2 \\
 5283.621 & 3.24 & -0.524 & 184.1 & 162.0 & 182.4 & 140.6 & 139.0 & 118.4 \\
 5302.302 & 3.28 & -0.880 & 152.1 & 129.4 & 148.3 & 145.9 & 129.7 & 178.3 \\
 5307.370 & 1.61 & -2.912 & 171.2 & 142.0 & 175.3 & 151.7 & 114.7 & 181.9 \\
 5324.190 & 3.21 & -0.100 & 192.4 & 183.4 & 182.2 & 182.3 & 180.1 & 191.2 \\
 5332.900 & 1.56 & -2.780 & 193.5 & 159.4 & 171.4 & 187.1 & 152.9 & 176.0 \\
 5339.930 & 3.27 & -0.720 & 150.4 & 131.9 & 157.4 & 154.2 & 119.6 & 160.0 \\
 5364.860 & 4.45 & 0.228 & 121.8 & 94.8 & 117.4 & 113.1 & 95.7 & 117.4 \\
 5367.480 & 4.42 & 0.443 & 110.2 & 105.2 & 126.2 & 133.3 & 108.5 & 136.8 \\
 5369.960 & 4.37 & 0.536 & 122.5 & 107.3 & 124.7 & 132.7 & 118.8 & 117.7 \\
 5383.370 & 4.31 & 0.645 & 147.6 & 134.9 & 166.2 & 148.2 & 145.6 & 154.0 \\
 5386.340 & 4.16 & -1.740 & \nodata & \nodata & \nodata & 39.5 & \nodata & 32.9 \\
 5389.480 & 4.42 & -0.400 & 97.8 & 76.1 & 92.6 & 50.8 & 66.5 & 79.8 \\
 5393.170 & 3.24 & -0.920 & 136.2 & 143.2 & 161.5 & 146.5 & 132.3 & 152.1 \\
 5395.220 & 4.45 & -1.730 & \nodata & \nodata & \nodata & \nodata & \nodata & 35.9 \\
 5400.510 & 4.37 & -0.150 & 100.0 & 89.1 & 115.4 & 102.4 & 98.0 & 91.2 \\
 5415.199 & 4.39 & 0.643 & 126.2 & 118.6 & 147.8 & 124.4 & 118.2 & 138.9 \\
 5424.070 & 4.32 & 0.520 & 161.7 & 134.5 & 151.4 & 141.3 & 141.5 & 113.2 \\
 5436.300 & 4.39 & -1.350 & \nodata & \nodata & 51.0 & 38.8 & \nodata & \nodata \\
 5464.280 & 4.14 & -1.402 & \nodata & \nodata & 30.8 & \nodata & 37.4 & \nodata \\
 5470.090 & 4.45 & -1.600 & \nodata & \nodata & \nodata & 30.5 & \nodata & 38.2 \\
 5497.516 & 1.01 & -2.825 & \nodata & \nodata & \nodata & \nodata & 169.4 & \nodata \\
 5501.465 & 0.96 & -3.046 & \nodata & \nodata & \nodata & \nodata & 185.0 & \nodata \\
 5506.790 & 0.99 & -2.789 & \nodata & 196.5 & \nodata & \nodata & 181.6 & \nodata \\
 5569.618 & 3.42 & -0.540 & 159.9 & 144.7 & 178.4 & 153.9 & 127.1 & 178.5 \\
 5572.842 & 3.40 & -0.310 & \nodata & 159.5 & 154.6 & \nodata & 129.9 & 167.8 \\
 5576.089 & 3.43 & -1.000 & 141.7 & 125.7 & \nodata & 150.2 & 112.7 & 172.0 \\
 5586.756 & 3.37 & -0.144 & 170.1 & 159.8 & 193.0 & 173.4 & 169.8 & 169.0 \\
 5615.660 & 3.33 & 0.050 & 187.5 & 172.7 & \nodata & 198.2 & 179.3 & 192.6 \\
 5624.540 & 3.42 & -0.755 & 142.8 & 130.5 & 141.9 & 141.5 & 112.5 & 130.5 \\
 5658.820 & 3.40 & -0.793 & 142.3 & 141.9 & 164.4 & 163.4 & 112.8 & 159.2 \\
 5662.516 & 4.18 & -0.573 & 83.2 & 87.5 & 116.0 & 90.4 & 71.3 & 68.3 \\
 5686.530 & 4.55 & -0.450 & 49.3 & 32.8 & 68.4 & 61.6 & \nodata & \nodata \\
 5701.543 & 2.56 & -2.143 & 128.8 & 120.7 & 141.3 & 134.1 & 115.4 & 132.5 \\
 5956.693 & 0.86 & -4.498 & 159.5 & 117.6 & 135.3 & 152.8 & 80.0 & 136.9 \\
 6003.030 & 3.88 & -1.110 & 87.6 & 36.3 & 91.7 & 102.6 & 34.3 & 73.1 \\
 6024.050 & 4.55 & -0.110 & 93.6 & 79.7 & 92.0 & 73.1 & 51.6 & 104.9 \\
 6027.048 & 4.07 & -1.089 & 62.6 & 36.2 & 68.4 & 75.2 & 36.4 & 44.0 \\
 6056.010 & 4.73 & -0.450 & 45.9 & 37.4 & 53.5 & 56.9 & \nodata & 35.3 \\
 6065.481 & 2.61 & -1.410 & 182.3 & \nodata & 179.0 & 164.0 & 144.5 & 126.4 \\
 6078.500 & 4.79 & -0.370 & 55.2 & 31.6 & 53.2 & 35.9 & 55.9 & 68.2 \\
 6079.010 & 4.65 & -0.950 & 32.5 & \nodata & \nodata & 48.2 & \nodata & 32.3 \\
 6082.720 & 2.22 & -3.548 & 67.4 & 50.6 & 71.7 & 73.1 & 52.0 & 46.3 \\
 6120.260 & 0.91 & -5.940 & 36.8 & \nodata & \nodata & 39.5 & \nodata & 40.1 \\
 6136.615 & 2.45 & -1.410 & 196.9 & \nodata & \nodata & 167.9 & 122.5 & 183.8 \\
 6136.992 & 2.20 & -2.932 & 138.6 & 98.9 & 131.4 & 131.2 & 107.5 & 96.4 \\
 6137.691 & 2.59 & -1.346 & 164.6 & 147.8 & 185.2 & 165.0 & 157.1 & 195.4 \\
 6151.619 & 2.18 & -3.371 & 88.7 & 71.5 & 96.3 & 92.3 & 61.4 & 72.3 \\
 6157.750 & 4.07 & -1.260 & 65.0 & \nodata & 67.2 & 55.9 & 41.5 & 64.8 \\
 6165.360 & 4.14 & -1.473 & \nodata & \nodata & \nodata & 32.7 & \nodata & \nodata \\
 6173.340 & 2.22 & -2.850 & 120.6 & 101.8 & 123.1 & 130.8 & 89.8 & 114.3 \\
 6180.203 & 2.73 & -2.649 & 68.1 & 55.3 & 74.2 & 65.5 & 53.2 & 69.1 \\
 6187.990 & 3.94 & -1.580 & 42.4 & \nodata & 42.4 & 40.4 & \nodata & 37.6 \\
 6191.558 & 2.43 & -1.416 & \nodata & 153.7 & 189.2 & 180.7 & 125.4 & \nodata \\
 6200.312 & 2.61 & -2.373 & 121.4 & 90.0 & 106.3 & 95.5 & 88.0 & 121.3 \\
 6213.430 & 2.22 & -2.481 & 142.8 & 101.5 & 126.0 & 139.2 & 109.9 & 132.0 \\
 6219.280 & 2.20 & -2.448 & 177.3 & 111.2 & 140.0 & \nodata & 127.6 & 143.4 \\
 6226.740 & 3.88 & -2.200 & \nodata & \nodata & 33.8 & 30.8 & \nodata & 35.2 \\
 6229.230 & 2.84 & -2.900 & 53.6 & 41.5 & 57.9 & 55.9 & \nodata & 36.3 \\
 6230.740 & 2.56 & -1.276 & 177.2 & \nodata & 179.5 & 186.3 & \nodata & \nodata \\
 6240.645 & 2.22 & -3.173 & 95.3 & 65.4 & 91.8 & 92.6 & 59.6 & 84.7 \\
 6246.320 & 3.60 & -0.733 & 136.5 & 103.4 & 120.3 & 110.9 & 98.5 & 85.0 \\
 6252.555 & 2.40 & -1.767 & 187.7 & 149.1 & 166.8 & 155.3 & 128.3 & 142.6 \\
 6254.260 & 2.28 & -2.443 & 151.9 & 133.8 & 152.6 & 124.0 & 99.2 & 154.2 \\
 6265.134 & 2.18 & -2.540 & 152.6 & 128.0 & 144.9 & 112.0 & 107.0 & 128.2 \\
 6290.970 & 4.73 & -0.760 & \nodata & \nodata & 46.4 & 36.8 & 35.5 & 45.1 \\
 6297.792 & 2.22 & -2.640 & 137.1 & 109.9 & 132.9 & 125.9 & 104.8 & 111.8 \\
 6301.500 & 3.65 & -0.720 & 109.9 & 103.4 & 105.3 & 117.7 & 99.0 & 93.0 \\
 6302.490 & 3.69 & -1.150 & 95.2 & 39.9 & 77.5 & 62.6 & \nodata & 60.7 \\
 6311.510 & 2.83 & -3.220 & 46.3 & \nodata & 55.8 & 44.1 & \nodata & 38.2 \\
 6322.684 & 2.59 & -2.469 & 133.8 & 90.2 & 85.1 & 122.4 & 60.5 & \nodata \\
 6330.850 & 4.73 & -1.220 & \nodata & \nodata & 30.4 & 34.2 & \nodata & \nodata \\
 6335.330 & 2.20 & -2.177 & 171.6 & 139.0 & 145.0 & 155.8 & 133.3 & 145.0 \\
 6336.820 & 3.69 & -1.050 & 101.1 & 92.4 & 91.6 & 109.8 & 98.0 & 93.6 \\
 6344.148 & 2.43 & -2.877 & 105.8 & 85.7 & 101.4 & 97.4 & 72.4 & 78.5 \\
 6355.029 & 2.84 & -2.291 & 99.6 & 86.8 & 93.9 & 97.1 & 78.2 & 95.5 \\
 6380.742 & 4.19 & -1.375 & 42.6 & \nodata & 49.1 & 35.3 & \nodata & 48.9 \\
 6392.540 & 2.28 & -3.950 & 39.2 & \nodata & 31.9 & 33.9 & \nodata & 48.3 \\
 6393.610 & 2.43 & -1.576 & 170.8 & 154.3 & 184.5 & \nodata & 132.5 & 136.1 \\
 6400.000 & 3.60 & -0.290 & 145.7 & 110.1 & 139.4 & 159.4 & 127.2 & 159.1 \\
 6408.030 & 3.69 & -1.000 & 103.6 & 78.1 & 102.2 & 108.4 & 70.1 & 105.7 \\
 6411.649 & 3.65 & -0.717 & 119.7 & 85.6 & 106.5 & 99.2 & 77.9 & 101.7 \\
 6419.960 & 4.73 & -0.240 & 61.9 & 48.1 & 74.9 & 58.4 & 50.2 & 49.9 \\
 6421.350 & 2.28 & -2.014 & 177.0 & 145.0 & \nodata & 139.1 & 144.0 & 143.1 \\
 6430.846 & 2.18 & -1.946 & 188.1 & \nodata & 176.5 & 163.8 & \nodata & \nodata \\
 6481.869 & 2.27 & -3.010 & 118.9 & 79.8 & 124.2 & 108.2 & 87.7 & 49.3 \\
 6494.980 & 2.40 & -1.239 & \nodata & 177.1 & \nodata & 191.2 & \nodata & 154.6 \\
 6498.940 & 0.96 & -4.689 & 142.6 & 106.3 & 130.0 & 114.3 & 100.3 & 94.0 \\
 6518.370 & 2.83 & -2.297 & 92.7 & 58.1 & 96.6 & 94.6 & 66.0 & 86.3 \\
 6533.930 & 4.55 & -1.460 & \nodata & \nodata & \nodata & \nodata & \nodata & 46.4 \\
 6574.228 & 0.99 & -5.022 & 108.1 & 78.3 & 114.1 & 115.7 & 49.3 & 73.5 \\
 6581.220 & 1.48 & -4.680 & 66.9 & \nodata & 75.1 & 55.3 & 46.9 & 58.3 \\
 6592.910 & 2.73 & -1.470 & 181.9 & 148.1 & \nodata & 144.2 & 130.3 & 188.9 \\
 6593.868 & 2.43 & -2.366 & 148.1 & 120.5 & 130.9 & 95.4 & 113.6 & 110.8 \\
 6597.560 & 4.79 & -1.070 & 32.8 & \nodata & 39.0 & \nodata & \nodata & 34.0 \\
 6608.030 & 2.28 & -3.940 & 46.9 & \nodata & 59.6 & 36.7 & \nodata & 56.4 \\
 6609.109 & 2.56 & -2.661 & 113.3 & 94.0 & 76.1 & 118.7 & 78.4 & 64.2 \\
 6627.540 & 4.54 & -1.680 & \nodata & \nodata & \nodata & \nodata & \nodata & 31.6 \\
 6633.748 & 4.56 & -0.799 & 40.9 & 36.4 & 46.9 & 56.7 & 32.9 & \nodata \\
 6663.440 & 2.42 & -2.479 & 144.7 & 79.2 & 134.9 & 135.5 & 64.7 & 106.3 \\
 6677.990 & 2.69 & -1.420 & 147.9 & \nodata & 193.0 & 184.7 & 152.7 & \nodata \\
 6750.150 & 2.42 & -2.621 & 84.4 & 110.3 & \nodata & 108.2 & 85.5 & 122.6 \\
\\
Fe II \\
 4923.920 & 2.89 & -1.320 & 170.3 & \nodata & 178.3 & 180.5 & 148.7 & 158.6 \\
 4993.350 & 2.81 & -3.620 & 55.0 & 45.7 & 75.8 & \nodata & 50.0 & 41.3 \\
 5018.430 & 2.89 & -1.220 & 188.0 & 189.2 & \nodata & 192.9 & 152.9 & 179.8 \\
 5197.570 & 3.23 & -2.100 & 114.5 & 102.3 & \nodata & 134.9 & 101.2 & 111.8 \\
 5234.630 & 3.22 & -2.118 & \nodata & 98.6 & 111.4 & 115.3 & \nodata & 94.1 \\
 5264.810 & 3.23 & -3.210 & 46.1 & 42.0 & 77.8 & 59.6 & 54.5 & 74.7 \\
 5276.000 & 3.20 & -1.950 & 138.2 & 124.8 & 156.6 & 150.3 & 115.9 & 105.6 \\
 5284.100 & 2.89 & -3.190 & 87.5 & 74.3 & 106.1 & 100.9 & 81.5 & \nodata \\
 5414.080 & 3.22 & -3.610 & \nodata & \nodata & 33.7 & 31.5 & 31.0 & \nodata \\
 5425.250 & 3.20 & -3.360 & 45.8 & 43.9 & 69.9 & 45.1 & 41.3 & 53.8 \\
 5534.850 & 3.24 & -2.920 & 69.0 & 71.5 & 104.9 & 76.4 & 80.2 & 80.0 \\
 5991.380 & 3.15 & -3.740 & \nodata & 35.1 & 38.5 & \nodata & \nodata & 50.3 \\
 6149.250 & 3.89 & -2.720 & \nodata & \nodata & 34.7 & \nodata & \nodata & \nodata \\
 6238.380 & 3.89 & -2.670 & 41.2 & 33.5 & 53.2 & 47.3 & 35.3 & 38.7 \\
 6247.560 & 3.89 & -2.360 & 46.5 & 39.5 & 51.5 & 39.0 & 39.2 & 68.7 \\
 6369.460 & 2.89 & -4.020 & \nodata & \nodata & 42.3 & \nodata & \nodata & 38.7 \\
 6416.930 & 3.89 & -2.790 & \nodata & \nodata & 53.9 & 45.1 & \nodata & 41.2 \\
 6432.680 & 2.89 & -3.710 & 41.9 & 43.7 & 66.2 & 33.7 & 45.5 & 52.9 \\
 6456.390 & 3.90 & -2.080 & 63.5 & 57.0 & 75.0 & 59.5 & 70.4 & 50.1 \\
 6516.080 & 2.89 & -3.450 & 60.7 & 58.6 & 85.6 & 80.9 & 60.2 & 54.8 \\
\\
O I \\
 6300.310 & 0.00 & -9.750 & 46.9 & 30.1 & $<$30.0 & 26.0 & 35.7 & $<$ 30.0 \\
\\
Na I \\
 5688.210 & 2.10 & -0.370 & 51.2 & $<$30.0 & $<$30.0 & 58.6 & 49.5 & 54.9 \\
\\
Mg I \\
 5528.410 & 4.34 & -0.480 & 179.4 & 168.1 & 142.4 & 185.9 & 170.9 & 165.6 \\
 5711.090 & 4.35 & -1.728 & 83.3 & 60.1 & 34.0 & 69.6 & 75.3 & 84.4 \\
\\
Si I \\
 5684.520 & 4.93 & -1.650 & \nodata & 52.0 & 39.0 & 41.3 & 33.1 & 32.4 \\
 6155.140 & 5.62 & -0.800 & \nodata & 32.9 & \nodata & \nodata & 37.3 & 35.7 \\
\\
Ca I \\
 5581.970 & 2.52 & -0.555 & 101.8 & 80.2 & 84.4 & 102.6 & 82.8 & 61.6 \\
 5588.749 & 2.52 & 0.210 & 150.1 & 142.7 & 138.1 & 150.0 & 152.1 & 134.5 \\
 5590.120 & 2.52 & -0.571 & 101.1 & 71.7 & 85.0 & 99.9 & 93.3 & 60.8 \\
 5594.470 & 2.52 & 0.097 & 141.6 & 129.2 & 129.4 & 143.7 & 142.0 & 113.2 \\
 5598.490 & 2.52 & -0.087 & 139.6 & 121.8 & \nodata & 109.4 & 128.1 & 132.1 \\
 5601.280 & 2.53 & -0.523 & 105.2 & 81.1 & 87.5 & 114.2 & 77.1 & 75.6 \\
 5857.451 & 2.93 & 0.230 & 121.9 & 66.3 & 96.8 & 112.0 & 92.2 & 115.6 \\
 6102.730 & 1.88 & -0.790 & 158.5 & 125.8 & 135.1 & 144.4 & 130.9 & 127.0 \\
 6122.230 & 1.89 & -0.320 & 178.6 & 162.8 & 171.6 & 182.5 & 121.1 & 162.8 \\
 6161.300 & 2.52 & -1.270 & 70.6 & 45.9 & 40.4 & 62.7 & 47.1 & 65.2 \\
 6162.173 & 1.90 & -0.090 & 197.0 & \nodata & 166.6 & 190.0 & 122.2 & \nodata \\
 6166.440 & 2.52 & -1.140 & 57.2 & 41.0 & 46.2 & 62.4 & 48.9 & 65.8 \\
 6169.040 & 2.52 & -0.800 & 107.5 & 65.5 & 61.5 & 92.7 & 75.9 & 55.7 \\
 6169.560 & 2.52 & -0.480 & 111.9 & 82.2 & 90.2 & 125.3 & 95.3 & 90.9 \\
 6439.080 & 2.52 & 0.390 & 186.2 & 143.7 & 157.3 & 151.4 & 139.2 & 175.7 \\
 6449.810 & 2.52 & -0.502 & 129.8 & 57.6 & 74.3 & 114.1 & 100.5 & 106.3 \\
 6455.600 & 2.52 & -1.290 & 63.8 & \nodata & 45.7 & 37.5 & 55.2 & 35.1 \\
 6471.670 & 2.52 & -0.760 & 93.8 & 70.8 & 87.5 & 89.6 & 55.8 & 68.3 \\
 6493.790 & 2.52 & -0.320 & \nodata & 83.0 & \nodata & \nodata & 82.5 & 101.5 \\
 6499.650 & 2.52 & -0.820 & 89.6 & 41.8 & 75.2 & 93.2 & 76.9 & 68.7 \\
 6717.681 & 2.71 & -0.610 & 81.5 & 60.4 & 74.6 & \nodata & 90.0 & 90.9 \\
\\
Sc II \\
 5031.021 & 1.36 & -0.400 & 131.9 & 101.6 & 60.5 & 125.3 & 114.0 & 91.7 \\
 5239.810 & 1.46 & -0.770 & 102.7 & 75.8 & 45.5 & 102.2 & 80.6 & 79.6 \\
 5318.370 & 1.36 & -2.010 & \nodata & \nodata & \nodata & 32.7 & \nodata & 30.8 \\
 5526.790 & 1.77 & 0.030 & 120.1 & 100.6 & 72.1 & 116.0 & 126.8 & 136.0 \\
 5641.000 & 1.50 & -1.130 & 60.6 & 46.7 & \nodata & 56.4 & 55.2 & 30.0 \\
 5657.910 & 1.51 & -0.600 & 106.8 & 91.1 & 80.0 & 111.6 & 108.9 & 111.0 \\
 5658.360 & 1.50 & -1.210 & 69.6 & \nodata & 34.7 & \nodata & 84.1 & 85.6 \\
 5667.160 & 1.50 & -1.310 & 65.5 & 45.6 & \nodata & 69.8 & 64.9 & 62.5 \\
 5669.060 & 1.50 & -1.200 & 78.0 & 61.0 & 36.3 & 82.9 & 48.1 & 78.1 \\
 5684.210 & 1.51 & -1.070 & 72.4 & 52.0 & 39.0 & 72.8 & 68.5 & 69.5 \\
 6245.620 & 1.51 & -0.970 & 79.8 & 49.0 & 31.9 & \nodata & 56.5 & 76.2 \\
 6309.900 & 1.50 & -1.520 & 41.1 & \nodata & \nodata & 31.6 & \nodata & 31.0 \\
 6604.580 & 1.36 & -1.310 & 62.4 & 43.3 & \nodata & 81.8 & 49.8 & 51.3 \\
\\
Ti I \\
 4840.870 & 0.90 & -0.450 & 135.2 & 88.2 & 93.3 & 118.9 & 98.7 & 123.1 \\
 4913.620 & 1.87 & 0.216 & 72.1 & 50.3 & 48.0 & 54.5 & 70.0 & 111.1 \\
 4981.731 & 0.84 & 0.500 & \nodata & 146.2 & 155.9 & \nodata & 123.1 & \nodata \\
 4991.065 & 0.84 & 0.380 & 190.9 & 144.4 & \nodata & 159.8 & 165.0 & \nodata \\
 4997.100 & 0.00 & -2.060 & 125.6 & 80.2 & 67.1 & 81.5 & 85.7 & 114.1 \\
 4999.503 & 0.83 & 0.250 & 188.4 & 154.2 & 139.4 & 185.4 & 146.5 & 146.4 \\
 5007.210 & 0.82 & 0.168 & 187.6 & \nodata & \nodata & \nodata & 156.9 & \nodata \\
 5009.650 & 0.02 & -2.203 & 121.7 & 50.0 & 43.2 & 80.5 & 60.4 & 90.3 \\
 5016.160 & 0.85 & -0.510 & 135.9 & 92.2 & 83.5 & 107.1 & 106.7 & 96.4 \\
 5020.020 & 0.84 & -0.358 & 135.5 & 92.0 & 91.6 & 126.1 & 87.3 & 125.5 \\
 5024.840 & 0.82 & -0.546 & 147.2 & 104.8 & 94.1 & 126.1 & 110.6 & 143.3 \\
 5035.900 & 1.46 & 0.260 & 154.9 & 89.5 & 108.6 & \nodata & 127.9 & 157.9 \\
 5036.460 & 1.44 & 0.186 & 129.7 & 94.6 & 98.2 & 114.8 & 102.1 & 119.0 \\
 5038.400 & 1.43 & 0.069 & 122.8 & 65.6 & 48.3 & 118.0 & 65.1 & 125.0 \\
 5039.957 & 0.02 & -1.130 & 181.6 & 123.0 & 128.9 & 128.8 & 129.4 & 167.0 \\
 5064.650 & 0.05 & -0.930 & 198.7 & 142.4 & 128.1 & 132.6 & 159.9 & 141.8 \\
 5113.440 & 1.44 & -0.727 & 52.3 & 30.4 & \nodata & 43.7 & \nodata & 48.6 \\
 5145.470 & 1.46 & -0.518 & 79.5 & 38.7 & \nodata & 48.8 & 51.6 & 61.6 \\
 5173.743 & 0.00 & -1.120 & \nodata & 145.3 & 141.6 & 171.3 & 141.2 & 172.7 \\
 5192.969 & 0.02 & -1.010 & \nodata & 164.2 & 150.0 & 189.6 & \nodata & \nodata \\
 5210.390 & 0.05 & -0.580 & 197.6 & 152.2 & \nodata & 157.5 & 144.2 & 179.5 \\
 5490.160 & 1.46 & -0.933 & 51.9 & \nodata & \nodata & 45.4 & 33.7 & 59.0 \\
 5978.540 & 1.87 & -0.440 & 42.5 & \nodata & \nodata & 39.1 & 33.2 & \nodata \\
 6126.220 & 1.07 & -1.425 & 65.0 & \nodata & \nodata & 53.8 & \nodata & 43.5 \\
 6258.100 & 1.44 & -0.355 & 106.0 & 48.4 & 39.5 & 69.9 & 69.0 & 57.0 \\
 6554.240 & 1.44 & -1.218 & 43.6 & \nodata & \nodata & 46.6 & \nodata & 38.0 \\
 6556.080 & 1.46 & -1.074 & 62.3 & \nodata & \nodata & 42.9 & 37.6 & 40.4 \\
 6599.130 & 0.90 & -2.090 & \nodata & \nodata & \nodata & \nodata & \nodata & 38.1 \\
 6743.130 & 0.90 & -1.630 & 61.2 & 33.0 & 35.5 & 46.8 & \nodata & 50.1 \\
\\
Ti II \\
 4798.530 & 1.08 & -2.670 & \nodata & \nodata & 72.8 & 94.4 & 84.2 & \nodata \\
 4805.090 & 2.06 & -1.120 & 126.8 & 114.9 & 110.3 & \nodata & 116.6 & \nodata \\
 4865.612 & 1.12 & -2.590 & 100.3 & 82.5 & 85.7 & 91.8 & \nodata & 129.4 \\
 4911.180 & 3.12 & -0.340 & 67.5 & 46.8 & \nodata & 74.8 & 45.3 & 50.4 \\
 5005.150 & 1.57 & -2.730 & 62.0 & 54.3 & 35.2 & 65.6 & \nodata & 66.9 \\
 5129.160 & 1.89 & -1.390 & 116.3 & 103.9 & 113.4 & \nodata & 114.2 & 119.8 \\
 5154.070 & 1.57 & -1.520 & 135.6 & 109.4 & 104.5 & 128.7 & 105.5 & 125.6 \\
 5185.913 & 1.89 & -1.350 & 112.3 & 88.5 & 85.6 & 91.7 & 101.8 & 110.5 \\
 5226.550 & 1.57 & -1.000 & 166.6 & 132.5 & 132.9 & 157.6 & 145.7 & 181.1 \\
 5268.610 & 2.60 & -1.620 & 42.8 & 30.8 & \nodata & \nodata & \nodata & 44.7 \\
 5336.771 & 1.58 & -1.700 & 126.0 & 101.6 & 108.8 & 117.5 & 122.1 & \nodata \\
 5381.010 & 1.57 & -1.780 & 115.9 & 107.0 & 93.0 & 117.8 & 86.0 & 155.5 \\
 5418.770 & 1.58 & -2.110 & 106.6 & 87.5 & 78.1 & 95.9 & 97.8 & 113.7 \\
 6219.940 & 2.06 & -2.820 & \nodata & \nodata & \nodata & \nodata & \nodata & 40.1 \\
 6559.588 & 2.05 & -2.019 & 60.3 & 30.5 & 35.8 & 50.2 & 51.5 & 53.6 \\
 6606.950 & 2.06 & -2.790 & \nodata & \nodata & \nodata & \nodata & \nodata & 44.1 \\
\\
V I \\
 6090.210 & 1.08 & -0.060 & 70.3 & \nodata & \nodata & 59.9 & 35.1 & 45.8 \\
 6119.530 & 1.06 & -0.320 & 55.3 & \nodata & \nodata & 54.9 & \nodata & 40.7 \\
 6135.370 & 1.05 & -0.750 & 31.5 & \nodata & \nodata & 32.2 & 36.6 & 46.1 \\
 6150.150 & 0.30 & -1.790 & 32.4 & \nodata & \nodata & 31.6 & \nodata & 32.4 \\
 6199.190 & 0.29 & -1.290 & 47.2 & \nodata & \nodata & 40.4 & 32.0 & 43.1 \\
 6216.360 & 0.28 & -0.810 & \nodata & \nodata & \nodata & \nodata & \nodata & 45.9 \\
 6224.510 & 0.29 & -2.010 & \nodata & \nodata & \nodata & \nodata & \nodata & 31.1 \\
 6233.200 & 0.28 & -2.070 & \nodata & \nodata & \nodata & 32.3 & \nodata & \nodata \\
 6243.110 & 0.30 & -0.980 & 84.6 & 43.9 & 33.9 & 74.0 & 56.0 & 65.9 \\
 6251.820 & 0.29 & -1.300 & 70.2 & \nodata & \nodata & 42.3 & \nodata & 54.4 \\
 6274.660 & 0.27 & -1.670 & 37.0 & 40.4 & \nodata & \nodata & 49.0 & 37.9 \\
 6285.160 & 0.28 & -1.560 & 49.6 & \nodata & \nodata & 41.7 & \nodata & \nodata \\
 6292.820 & 0.29 & -1.520 & 57.3 & \nodata & \nodata & 42.3 & \nodata & 31.5 \\
\\
Cr I \\
 5247.560 & 0.96 & -1.640 & 146.7 & 109.6 & 120.8 & 111.2 & 110.4 & 151.4 \\
 5345.801 & 1.00 & -0.980 & 186.6 & 152.3 & 150.3 & 148.6 & 129.0 & \nodata \\
 5409.800 & 1.03 & -0.720 & 186.1 & 149.9 & 174.8 & 155.3 & 156.1 & 190.8 \\
 6330.093 & 0.94 & -2.920 & 65.3 & 37.2 & 61.0 & 71.3 & 52.2 & 55.3 \\
%\\
%Cr II \\
% 4824.130 & 3.87 & -1.230 & 87.2 & \nodata & \nodata & \nodata & 50.3 & 60.2 \\
% 4848.240 & 3.86 & -1.130 & 66.1 & 59.2 & 75.5 & 72.2 & 33.1 & 55.8 \\
\\
Mn I \\
 4823.524 & 2.32 & 0.140 & 161.7 & 128.5 & 138.1 & 137.3 & 145.9 & 112.1 \\
 5407.420 & 2.14 & -1.743 & 53.3 & \nodata & 57.2 & 74.5 & \nodata & 32.9 \\
 5420.360 & 2.14 & -1.460 & 79.1 & 37.5 & 65.6 & 72.5 & 74.8 & \nodata \\
 5432.550 & 0.00 & -3.795 & 141.4 & 86.3 & 134.5 & 128.3 & 76.3 & 92.0 \\
 5516.770 & 2.18 & -1.847 & 30.5 & \nodata & \nodata & 38.0 & 34.8 & \nodata \\
 6013.510 & 3.07 & -0.252 & 64.4 & \nodata & 47.2 & 52.2 & \nodata & 42.5 \\
 6021.820 & 3.08 & 0.035 & 90.7 & 39.1 & 38.5 & 69.9 & 50.7 & 80.3 \\
\\
Co I \\
 5483.340 & 1.71 & -1.488 & 93.6 & 41.6 & $<$30.0 & 80.2 & 59.4 & 88.0 \\
 5647.230 & 2.28 & -1.560 & \nodata & \nodata & \nodata & \nodata & \nodata & 32.0 \\
\\
Ni I \\
 4855.410 & 3.54 & 0.000 & \nodata & 97.0 & 82.2 & 112.9 & 98.8 & 81.1 \\
 4980.160 & 3.61 & 0.070 & 105.6 & 72.2 & 67.0 & 102.1 & \nodata & 122.2 \\
 5017.590 & 3.54 & -0.080 & 87.8 & 53.2 & 56.1 & 97.3 & 73.3 & 82.9 \\
 5035.370 & 3.63 & 0.290 & 96.4 & 79.6 & 89.1 & 109.2 & 85.8 & 131.5 \\
 5080.520 & 3.65 & 0.130 & 96.3 & 81.7 & 86.0 & 104.4 & 85.1 & 81.1 \\
 5084.080 & 3.68 & 0.030 & 74.0 & 61.4 & 56.5 & 81.9 & 51.7 & 84.9 \\
 5137.070 & 1.68 & -1.990 & 151.9 & 109.3 & \nodata & 131.3 & 122.0 & 139.3 \\
 5476.920 & 1.83 & -0.890 & \nodata & 179.2 & 173.9 & 188.1 & 176.0 & 193.9 \\
 5578.730 & 1.68 & -2.670 & 106.0 & 73.4 & 86.2 & 122.9 & 72.2 & 95.4 \\
 5587.870 & 1.93 & -2.370 & 100.1 & 57.3 & 84.1 & 84.9 & 72.7 & 96.9 \\
 6128.970 & 1.68 & -3.390 & 44.9 & 31.4 & \nodata & 52.1 & \nodata & 40.1 \\
 6176.820 & 4.09 & -0.430 & 40.2 & \nodata & \nodata & 30.6 & \nodata & 38.0 \\
 6327.600 & 1.68 & -3.090 & 59.5 & 55.4 & 40.5 & 67.1 & 45.0 & 63.7 \\
 6482.800 & 1.94 & -2.850 & 61.5 & 41.6 & 52.3 & 70.2 & 50.4 & 49.3 \\
 6586.320 & 1.95 & -2.790 & 55.9 & 44.0 & 40.4 & 75.1 & \nodata & 56.5 \\
 6643.640 & 1.68 & -2.300 & 152.4 & \nodata & 115.3 & 126.5 & 113.9 & 113.2 \\
 6767.780 & 1.83 & -2.170 & 137.6 & \nodata & 104.3 & 120.9 & 103.5 & 90.0 \\
\\
Cu I \\
 5105.500 & 1.39 & -1.505 & 115.5 & 50.1 & $<$30.0 & 89.6 & 71.8 & \nodata \\
\\
Zn I \\
 4810.540 & 4.08 & -0.170 & 85.2 & 58.2 & 41.7 & 81.7 & 81.2 & 60.0 \\
\\
Y II \\
 4883.690 & 1.08 & 0.070 & 118.9 & 79.6 & 42.6 & 86.9 & 99.4 & 121.7 \\
 5087.430 & 1.08 & -0.170 & 79.9 & 63.2 & 37.0 & 76.3 & 66.4 & 90.0 \\
 5200.420 & 0.99 & -0.570 & 61.8 & 56.6 & $<$30.0 & \nodata & 60.8 & 77.9 \\
\\
Ba II \\
 5853.690 & 0.60 & -1.010 & 152.0 & 137.6 & 93.0 & 92.7 & 121.7 & 130.0 \\
 6141.730 & 0.70 & -0.077 & \nodata & \nodata & S & 144.9 & 162.0 & S \\
 6496.910 & 0.60 & -0.380 & \nodata & \nodata & 163.0 & 173.6 & 159.5 & 195.0 \\
\\
La II \\
 6320.430 & 0.17 & -1.562 & 45.1 & 37.2    & $<$30.0 & $<$30.0 & $<$30.0 & $<$30.0 \\
 6390.460 & 0.32 & -1.400 & 41.2 & $<$30.0 & $<$30.0 & $<$30.0 & $<$30.0 & $<$30.0 \\
 6774.270 & 0.13 & -1.708 & 42.8 & 31.0    & $<$30.0 & $<$30.0 & 36.0    & $<$30.0 \\
\\
Nd II \\
 5249.590 & 0.98 & 0.200 & 84.8 & 70.3 & $<$30.0 & 77.1 & 48.3 & 52.1 \\
 5319.820 & 0.55 & -0.140 & 99.5 & 70.9 & 30.6 & 67.1 & 48.2 & 80.3 \\
\\
Eu II \\
 6645.130 & 1.37 & 0.120 & 30.5 & $<$30.0 & $<$30.0 & $<$30.0 & $<$30.0 & 34.4 \\
%\enddata
%\tablecomments{  }
%\end{deluxetable}
\end{longtable}

